VeraSel: Verifiable Random Selection for Mixnets Construction

The security and performance of Mixnets depends on the trustworthiness of the Mixnodes in the network. The challenge is to limit the adversary's influence on which Mixnodes operate in the network. A trusted party (such as the Mixnet operator) may ensure this, however, it is a single point of failure in the event of corruption or coercion. Therefore, we study the problem of how to select a subset of Mixnodes in a distributed way for Mixnet construction. We present VeraSel, a scheme that enables Mixnodes to be chosen according to their weights in a distributed, unbiased, and verifiable fashion using Verifiable Random Functions (VRFs). It is shown that VeraSel enables any party to learn and verify which nodes has been selected based on the commitments and proofs generated by each Mixnode with VRF.

==> 3_model.tex <==
\section{Threat Model--0.5 page}
\label{sec:threat model}


